An Internal Model Principle For Robots

When designing a robot's internal system, one often makes assumptions about the structure of the intended environment of the robot. One may even assign meaning to various internal components of the robot in terms of expected environmental correlates. In this paper we want to make the distinction between robot's internal and external worlds clear-cut. Can the robot learn about its environment, relying only on internally available information, including the sensor data? Are there mathematical conditions on the internal robot system which can be internally verified and make the robot's internal system mirror the structure of the environment? We prove that sufficiency is such a mathematical principle, and mathematically describe the emergence of the robot's internal structure isomorphic or bisimulation equivalent to that of the environment. A connection to the free-energy principle is established, when sufficiency is interpreted as a limit case of surprise minimization. As such, we show that surprise minimization leads to having an internal model isomorphic to the environment. This also parallels the Good Regulator Principle which states that controlling a system sufficiently well means having a model of it. Unlike the mentioned theories, ours is discrete, and non-probabilistic.

==> Robot_arm_ex.tex <==
\section{Example: Robot Arm}
\textbf{Lemma} The semiautomaton system of the robot arm is \textit{minimally distinguishing}. 

\textit{proof.} 
Let $e \in X$ denotes a configuration of the robot arm determined by the directions $\theta_1, \theta_2, \cdots, \theta_n$. Let $A$ be a set of continuous and order-preserving actions. We need to show that for all actions $a \in A$ and for all $e_0, e_1, e_2 \in X$, we have the following: if $\tau(e_1,a) = \tau(e_2,a) = e_0$, then one of the following holds: $e_0 = e_1, e_1 = e_2$, or $e_0 = e_2$. 

\textbf{Injectivity of $\tau$ given a:}
For a fixed action $a$, the function $\tau(.,a): X \rightarrow X$ maps states in X to states in X. If $\tau(e_1,a) = \tau(e_2,a) = e_0$, then $e_1$ must equal $e_2$ due to the nature of the state space $X$ (which is homomorphic to $(S^1)^n)$. This is because in the $n$-torus, each state (set of directions) uniquely determines the configuration. 
Hence, by injectivity of $\tau$, $\tau(e_1,a) = \tau(e_2,a) = e_0$ implies $e_1 = e_2$, and this concludes the proof. 

Action $a$ is order-preserving if:
\begin{align}
    \forall \theta_1,\theta_2 \in [0,2\pi), \theta_1 < \theta_2 \rightarrow \tau(\theta_1,a) < \tau(\theta_2,a).
\end{align}


==> bib.tex <==
\begin{thebibliography}{8}
@article{autonomy2020,
  title={Autonomy and metrics of autonomy},
  author={Antsaklis, Panos},
  journal={Annual Reviews in Control},
  volume={49},
  pages={15--26},
  year={2020},
  publisher={Elsevier}
}


@article{ConAsh70,
    author={R. C. Conant and W. R. Ashby},
    title={Every good regulator of a system must be a model of that system},
    volume={1},
    number={2},
    journal={International Journal of Systems Science}, 
    year={1970},
    pages={89–97} }

@article{FraWon76,
    author={Francis, B.A. and Wonham, W.M.},
    title={The internal model principle of control theory}, volume={12},
    number={5},
    journal={Automatica},
    year={1976},
    pages={457–465} }


@article{Fri12,
    author={K. Friston},
    title={A free energy principle for biological systems}, volume={14},
    number={11},
    journal={Entropy},
    year={2012},
    pages={2100–2121} }

@article{RamFriHip20,
    author={M. J. D. Ramstead and K. J. Friston and I. Hip\'{o}lito},
    title={Is the Free-Energy Principle a Formal Theory of Semantics? From Variational Density Dynamics to Neural and Phenotypic Representations},
    volume={22},
    number={8},
    journal={Entropy},
    year={2020},
    pages={889} }


@book{ParPezFri22,
    author={T. Parr and G. Pezzulo and K. J. Friston},
    title={Active inference: The Free Energy Principle in Mind, Brain and Behaviour},
    journal={The MIT Press},
    year={2022}}

@article{HeiMilDaCManFriCou24,
    author={C. Heins and B. Millidge and L. Da Costa and R. P. Mann and K. J. Friston  and I. D. Couzin},
    title={Collective behavior from surprise minimization}, volume={121},
    number={17},
    journal={Proceedings of the National Academy of Sciences of the United States of America},
    year={2024} }


@book{reinforcement2018,
  title={Reinforcement Learning, second edition: An Introduction},
  author={Sutton, R.S. and Barto, A.G.},
  isbn={9780262352703},
  series={Adaptive Computation and Machine Learning series},
  url={https://books.google.fi/books?id=uWV0DwAAQBAJ},
  year={2018},
  publisher={MIT Press}
}
@INBOOK{MDPRL,
  author={Hoang, Dinh Thai and Huynh, Nguyen Van and Nguyen, Diep N. and Hossain, Ekram and Niyato, Dusit},
  booktitle={Deep Reinforcement Learning for Wireless Communications and Networking: Theory, Applications and Implementation}, 
  title={Markov Decision Process and Reinforcement Learning}, 
  year={2023},
  volume={},
  number={},
  pages={25-36},
  doi={10.1002/9781119873747.ch2}}

@InProceedings{FullMDPZhang,
  title = 	 {Making Linear {MDP}s Practical via Contrastive Representation Learning},
  author =       {Zhang, Tianjun and Ren, Tongzheng and Yang, Mengjiao and Gonzalez, Joseph and Schuurmans, Dale and Dai, Bo},
  booktitle = 	 {Proceedings of the 39th International Conference on Machine Learning},
  pages = 	 {26447--26466},
  year = 	 {2022},
  volume = 	 {162},
  month = 	 {17--23 Jul},
  publisher =    {PMLR},
  pdf = 	 {https://proceedings.mlr.press/v162/zhang22x/zhang22x.pdf},
  url = 	 {https://proceedings.mlr.press/v162/zhang22x.html}
}

@article{FullMDPRen,
  title={Spectral Decomposition Representation for Reinforcement Learning},
  author={Tongzheng Ren and Tianjun Zhang and Lisa Lee and Joseph E. Gonzalez and Dale Schuurmans and Bo Dai},
  journal={ArXiv},
  year={2022},
  volume={abs/2208.09515},
  url={https://api.semanticscholar.org/CorpusID:251719318}
}
@INPROCEEDINGS{POMDPChen,
  author={Chen, Min and Frazzoli, Emilio and Hsu, David and Lee, Wee Sun},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)}, 
  title={POMDP-lite for robust robot planning under uncertainty}, 
  year={2016},
  volume={},
  number={},
  pages={5427-5433},
  keywords={Robots;Bayes methods;Uncertainty;Markov processes;Games;Planning;Observability},
  doi={10.1109/ICRA.2016.7487754}}
@article{POMDPHanna,
   author = "Kurniawati, Hanna",
   title = "Partially Observable Markov Decision Processes and Robotics", 
   journal= "Annual Review of Control, Robotics, and Autonomous Systems",
   year = "2022",
   volume = "5",
   number = "Volume 5, 2022",
   pages = "253-277",
   doi = "https://doi.org/10.1146/annurev-control-042920-092451",
   url = "https://www.annualreviews.org/content/journals/10.1146/annurev-control-042920-092451",
   publisher = "Annual Reviews",
   issn = "2573-5144",
   type = "Journal Article"
  }
@article{KnownEnvJana,
title = {Multi-agent planning under local LTL specifications and event-based synchronization},
journal = {Automatica},
volume = {70},
pages = {239-248},
year = {2016},
issn = {0005-1098},
doi = {https://doi.org/10.1016/j.automatica.2016.04.006},
url = {https://www.sciencedirect.com/science/article/pii/S0005109816301285},
author = {Jana Tumova and Dimos V. Dimarogonas}
}
@ARTICLE{KnownEnvKantaros,
  author={Kantaros, Yiannis and Zavlanos, Michael M.},
  journal={IEEE Transactions on Automatic Control}, 
  title={Sampling-Based Optimal Control Synthesis for Multirobot Systems Under Global Temporal Tasks}, 
  year={2019},
  volume={64},
  number={5},
  pages={1916-1931},
  doi={10.1109/TAC.2018.2853558}}
@INPROCEEDINGS{UnknownEnvDorsa,
  author={Sadigh, Dorsa and Kim, Eric S. and Coogan, Samuel and Sastry, S. Shankar and Seshia, Sanjit A.},
  booktitle={53rd IEEE Conference on Decision and Control}, 
  title={A learning based approach to control synthesis of Markov decision processes for linear temporal logic specifications}, 
  year={2014},
  volume={},
  number={},
  pages={1091-1096},
  keywords={Bismuth;Markov processes;Vehicles;Automata;Safety;Learning (artificial intelligence);Process control},
  doi={10.1109/CDC.2014.7039527}}
@article{DRLKai,
  title={Deep reinforcement learning: A brief survey},
  author={Arulkumaran, Kai and Deisenroth, Marc Peter and Brundage, Miles and Bharath, Anil Anthony},
  journal={IEEE Signal Processing Magazine},
  volume={34},
  number={6},
  pages={26--38},
  year={2017},
  publisher={IEEE}
}
@article{DRLPablo,
  title={Active inference in robotics and artificial agents: Survey and challenges},
  author={Lanillos, Pablo and Meo, Cristian and Pezzato, Corrado and Meera, Ajith Anil and Baioumy, Mohamed and Ohata, Wataru and Tschantz, Alexander and Millidge, Beren and Wisse, Martijn and Buckley, Christopher L and others},
  journal={arXiv preprint arXiv:2112.01871},
  year={2021}
}

\end{thebibliography}
